Transactions Make Debugging Easy

We propose TROD, a novel transaction-oriented framework for debugging modern distributed web applications and online services. Our critical insight is that if applications store all state in databases and only access state transactionally, TROD can use lightweight always-on tracing to track the history of application state changes and data provenance, and then leverage the captured traces and transaction logs to faithfully replay or even test modified code retroactively on any past event. We demonstrate how TROD can simplify programming and debugging in production applications, list several research challenges and directions, and encourage the database and systems communities to drastically rethink the synergy between the way people develop and debug applications.

==> prototype.tex <==
\section{Proof of Concept}
\label{sec:prototype}

Use the case study example to construct the application and bug in our new environment.
Show some numbers of how fast Postgres/MySQL can make Point-in-Time Recovery, and how much storage space it would take. A few experiments and numbers here.

Then show that we can re-execute by running GDB or adding more log statements while repeatedly replaying the execution.
Multi-level debugging.
We do not need to capture every instruction for reproducing a function, as long as we can capture the transaction information.
